A model of stochastic memoization and name generation in probabilistic programming: categorical semantics via monads on presheaf categories

Stochastic memoization is a higher-order construct of probabilistic programming languages that is key in Bayesian nonparametrics, a modular approach that allows us to extend models beyond their parametric limitations and compose them in an elegant and principled manner. Stochastic memoization is simple and useful in practice, but semantically elusive, particularly regarding dataflow transformations. As the naive implementation resorts to the state monad, which is not commutative, it is not clear if stochastic memoization preserves the dataflow property -- i.e., whether we can reorder the lines of a program without changing its semantics, provided the dataflow graph is preserved. In this paper, we give an operational and categorical semantics to stochastic memoization and name generation in the context of a minimal probabilistic programming language, for a restricted class of functions. Our contribution is a first model of stochastic memoization of constant Bernoulli functions with a non-enumerable type, which validates data flow transformations, bridging the gap between traditional probability theory and higher-order probability models. Our model uses a presheaf category and a novel probability monad on it.

==> probabilistic-local-state-monad.tex <==
\section{Probabilistic local state monad}

\begin{definition}[Probabilistic local state monad]
    For all covariant presheaf $X：\BiG → \Sets$ and bigraph $g ∈ \BiG$:
    \[
    T(X)(g) \,≝\, \bigg(\Prfin \int^{g ↪ h} \Big( X(h)\times [0, 1]^{(h-g)_L}\Big)\bigg)^{[0,1]^{g_L}}
\]
\end{definition}


It is similar to the read-only state monad, except that any fresh node can be initialized. Every $λ ∈ [0, 1]^{g_L}$ is thought of as the probability of the corresponding function/left node being true on a new fresh atom. We will refer to such a $λ$ as a \emph{state of biases}.

The coend takes care of garbage collection. Indeed, if $g$ is a subbigraph of $h, h'$, and $h$ is a subbigraph of $h'$, by universal property of the coend, we have the following commutative diagram:  
    % https://q.uiver.app/?q=WzAsNCxbMSwwLCJYKGgpIMOXIFswLCAxXV57KGgnIC1nKV9MfSJdLFswLDEsIlgoaCcpIMOXIFswLCAxXV57KGgnIC1nKV9MfSJdLFsyLDEsIlgoaCkgw5cgWzAsIDFdXnsoaCAtZylfTH0iXSxbMSwyLCJcXGludF57Z1xcdG8gaH0gXFxCaWcoIFgoaClcXHRpbWVzIFswLCAxXV57KGgtZylfTH1cXEJpZykiXSxbMCwxLCJYKGgg4oaqIGgnKSDDlyAxIiwyXSxbMCwyLCIxIMOXICgtIFxcY2lyYyAoaC1nKV9MIOKGqiAoaCctZylfTCkgIl0sWzEsM10sWzIsM11d
\[\begin{tikzcd}
    & {X(h) × [0, 1]^{(h' -g)_L}} \\
    {X(h') × [0, 1]^{(h' -g)_L}} && {X(h) × [0, 1]^{(h -g)_L}} \\
    & {\int^{g ↪ h} \Big( X(h)\times [0, 1]^{(h-g)_L}\Big)}
    \arrow["{X(h ↪ h') × 1}"', from=1-2, to=2-1]
    \arrow["{1 × (- \circ (h-g)_L ↪ (h'-g)_L) }", from=1-2, to=2-3]
    \arrow[from=2-1, to=3-2]
    \arrow[from=2-3, to=3-2]
\end{tikzcd}\]
This means that if the state of biases is defined over $h'$ but $h'-h$ is unused (since the program comes from an element $X(h)$), we might as well discard it and restrict ourselves to $h$ (\ie $h'-h$ is garbage collected).

In the following subsections, we will show that:

\begin{theorem}
The assignment $T$ can be extended to an affine strong commutative monad on $\BiG$. 
\end{theorem}

%TODO: And ideally this is a submonad on the monad of all probability measure on $\Sets^{\BiG}$ (or a sheaf subtopos).

\subsection{Functoriality}

In the following, $X, Y, Z：\BiG → \Sets$ denote presheaves, $g = (g_L, g_R, E^g), g', h, h' ∈ \BiG$ bigraphs, $ι, ι'：g ↪ g'$ bigraph embeddings, and $λ, λ'：[0, 1]^{g_L}$ states of biases. We will omit subscripts when they are clear from the context.

Equivalence classes in $\int^{g ↪ h} X(h)\times [0, 1]^{(h-g)_L}$ are written $[x_h, λ^h]_g$. We use Dirac's bra-ket notation $\Ket{[x_h, λ^h]_g}_h$ to denote a formal column vector of equivalence classes ranging over a finite set of $h$'s. As such, a formal convex sum $\sum_i p_i [x_{h_i}, λ^{h_i}]_g ∈ \Prfin \int^{g ↪ h} X(h)\times [0, 1]^{(h-g)_L}$ will be concisely denoted by $\Braket {\vec p | [x_h, λ^h]_g}_h$.

\begin{definition}[Action of $T(X)$ on morphisms] 
    \[
    T(X)(g \xinjto {ι} g')：\\
    \begin{cases}
    \displaystyle\Big(\Prfin \int^{g ↪ h} \mkern-30mu X(h)\times [0, 1]^{(h-g)_L}\Big)^{[0,1]^{g_L}}
    ⟶ \Big(\Prfin \int^{g' ↪ h'} \mkern-35mu X(h')\times [0, 1]^{(h'-g')_L}\Big)^{[0,1]^{g'_L}} \span\\
    ϑ ↦ [0,1]^{g'_L} \xto {- \circ ι_L} [0,1]^{g_L} &\xto {ϑ} \Prfin \displaystyle\int^{g ↪ h} X(h)\times [0, 1]^{(h-g)_L} \\
    &\xto{\Prfin ψ_{g, g'}} \Prfin \displaystyle\int^{g' ↪ h'} X(h')\times [0, 1]^{(h'-g')_L}
    \end{cases}
    \]
    where 
    
    \begin{itemize}
        \item the map $\int^{g ↪ h} X(h)\times [0, 1]^{(h-g)_L} \xto{ψ_{g, g'}} \int^{g' ↪ h'} X(h')\times [0, 1]^{(h'-g')_L}$ is given by:\,\\[1em] 
        \begin{prooftree}
            \hypo{\begin{cases}
                X(h)\times [0, 1]^{(h-g)_L} → X(h \pushout_g g')\times [0, 1]^{(h \pushout_g g' - g')_L} → \mathrlap{\int^{g' ↪ h'} X(h')\times [0, 1]^{(h'-g')_L}}\\
                (x_h, \, λ^h) ⟼ (X(h ↪ h \pushout_g g')(x_h), \, λ^h) ⟼ \mathrlap{[X(h ↪ h \pushout_g g')(x_h), \, λ^h]_{g'}}\vphantom{\bigg|}
            \end{cases}}
            \infer1[extranat. in $h$]{\int^{g ↪ h} X(h)\times [0, 1]^{(h-g)_L} \xto{ψ_{g, g'}} \int^{g' ↪ h'} X(h')\times [0, 1]^{(h'-g')_L}}
        \end{prooftree}\\[1em]
    \item $ι_L：g_L ↪ g_L'$ is the embedding restricted to left nodes.
    \item $h \pushout_g g'$ is the pushout in the category of graphs regarded as an object of $\BiG$:
    % https://q.uiver.app/?q=WzAsNCxbMCwwLCJnIl0sWzEsMCwiZyciXSxbMCwxLCJoIl0sWzEsMSwiaCBcXGNvcHJvZF9nIGcnIl0sWzAsMSwiIiwwLHsic3R5bGUiOnsidGFpbCI6eyJuYW1lIjoiaG9vayIsInNpZGUiOiJ0b3AifX19XSxbMCwyLCIiLDIseyJzdHlsZSI6eyJ0YWlsIjp7Im5hbWUiOiJob29rIiwic2lkZSI6InRvcCJ9fX1dLFsyLDMsIiIsMix7InN0eWxlIjp7InRhaWwiOnsibmFtZSI6Imhvb2siLCJzaWRlIjoidG9wIn19fV0sWzEsMywiIiwwLHsic3R5bGUiOnsidGFpbCI6eyJuYW1lIjoiaG9vayIsInNpZGUiOiJ0b3AifX19XSxbMywwLCIiLDEseyJzdHlsZSI6eyJuYW1lIjoiY29ybmVyIn19XV0=
    \[\begin{tikzcd}
        g & {g'} \\
        h & {h \pushout_g g'}
        \arrow[hook, from=1-1, to=1-2]
        \arrow[hook, from=1-1, to=2-1]
        \arrow[hook, from=2-1, to=2-2]
        \arrow[hook, from=1-2, to=2-2]
        \arrow["\lrcorner"{anchor=center, pos=0.125, rotate=180}, draw=none, from=2-2, to=1-1]
    \end{tikzcd}\]
    \end{itemize}
    
    More concretely, with Dirac's convenient bra-ket notation, $T(X)(g \xinjto {ι} g')$ can be written as:
    \[
    T(X)(ι) =
    \begin{cases}
        \Big(\Prfin \int^{g ↪ h} X(h)\times [0, 1]^{(h-g)_L}\Big)^{[0,1]^{g_L}}
        ⟶ \Big(\Prfin \int^{g' ↪ h'} X(h')\times [0, 1]^{(h'-g')_L}\Big)^{[0,1]^{g'_L}} \\
        ϑ ⟼ λ' ↦ \letin{ϑ(λ'ι_L)}{\Braket {\vec p | [x_h, λ^h]_g}_h}{\Braket {\vec p | [X(h ↪ h \pushout_g g')(x_h), λ^h]_{g'}}_h}
    \end{cases}
    \]
\end{definition}

In the definition of $ψ_{g, g'}$, extranaturality in $h$ does indeed hold, as for every $g ↪ h_1, h_2$ and $h_1 ↪ h_2$:

\adjustbox{scale=.7,center}{%
% https://q.uiver.app/?q=WzAsMTAsWzIsMCwiWChoXzEpIMOXIFswLCAxXV57KGhfMiAtIGcpX0x9Il0sWzIsMSwieF8xLCDOu18yIl0sWzMsMiwiWChoXzEg4oaqIGhfMikoeF8xKSwgzrtfMiJdLFsxLDIsInhfMSwgzrtfMs65J19MIl0sWzIsMywiW1goaF8xIOKGqiBoXzEgXFxjb3Byb2RfZyBnJykoeF8xKSwgzrtfMs65J19MXV97Zyd9Il0sWzIsNCwiW1goXFx1bmRlcmJyYWNle2hfMSBcXCzihqpcXCwgaF8yIFxcO+KGqlxcOyBoXzIgXFx0ZXh0c3R5bGVcXGNvcHJvZF9nIGcnfV97PSBcXDsgaF8xIOKGqiBoXzEgXFxzY3JpcHRzdHlsZVxcY29wcm9kX2cgZycg4oaqIGhfMiBcXHNjcmlwdHN0eWxlXFxjb3Byb2RfZyBnJ30pKHhfMSksIM67XzJdX3tnJ30iXSxbMCwyLCJYKGhfMSkgw5cgWzAsIDFdXnsoaF8xIC0gZylfTH0iXSxbNCwyLCJYKGhfMikgw5cgWzAsIDFdXnsoaF8yIC0gZylfTH0iXSxbMiw1LCJcXGludF57ZydcXHRvIGgnfSBYKGgnKVxcdGltZXMgWzAsIDFdXnsoaCctZycpX0x9Il0sWzQsNV0sWzEsMl0sWzEsM10sWzMsNF0sWzIsNV0sWzQsNSwiIiwyLHsic2hvcnRlbiI6eyJzb3VyY2UiOjIwLCJ0YXJnZXQiOjIwfSwibGV2ZWwiOjIsInN0eWxlIjp7ImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbMCw2XSxbMCw3XSxbNiw4LCIiLDIseyJjdXJ2ZSI6M31dLFs3LDgsIiIsMSx7ImN1cnZlIjotM31dXQ==
\begin{tikzcd}
	&& {X(h_1) × [0, 1]^{(h_2 - g)_L}} \\
	&& {x_1, λ_2} \\
	{X(h_1) × [0, 1]^{(h_1 - g)_L}} & {x_1, λ_2ι'_L} && {X(h_1 ↪ h_2)(x_1), λ_2} & {X(h_2) × [0, 1]^{(h_2 - g)_L}} \\
	&& {[X(h_1 ↪ h_1 \coprod_g g')(x_1), λ_2ι'_L]_{g'}} \\
	&& {[X(\underbrace{h_1 \,↪\, h_2 \;↪\; h_2 \textstyle\coprod_g g'}_{= \; h_1 ↪ h_1 \scriptstyle\coprod_g g' ↪ h_2 \scriptstyle\coprod_g g'})(x_1), λ_2]_{g'}} \\
	&& {\int^{g' ↪ h'} X(h')\times [0, 1]^{(h'-g')_L}} && {}
	\arrow[from=2-3, to=3-4]
	\arrow[from=2-3, to=3-2]
	\arrow[from=3-2, to=4-3]
	\arrow[from=3-4, to=5-3]
	\arrow[shorten <=2pt, shorten >=2pt, Rightarrow, no head, from=4-3, to=5-3]
	\arrow[from=1-3, to=3-1]
	\arrow[from=1-3, to=3-5]
	\arrow[curve={height=18pt}, from=3-1, to=6-3]
	\arrow[curve={height=-18pt}, from=3-5, to=6-3]
\end{tikzcd}
}


\begin{proposition}[Functoriality]
    $T$ is an endofunctor on $\BiG$. 
\end{proposition}

\begin{proof}
    For $ι：g ↪ g = \id$, $\Braket {\vec p | [X(h ↪ \smash{ \underbrace{h \textstyle\pushout_g g}_{= \, h}})(x_h), λ^h]_{g}}_h = \Braket {\vec p | [x_h, λ^h]_{g'}}_h$ and $λ' ι_L = λ'$ so $T(X)(g \xinjto {ι} g) = \id$.

    For every $g ↪ g' ↪ g''$:
    \begin{multline*}
        \sum\limits_{ i } {\textstyle p_i \Big[X(h_i ↪ h_i \pushout_g g'')(x_{h_i}), λ^{h_i}\Big]_{g''}} \\
        =
        \sum\limits_{ i } {\textstyle  p_i \Big[X(h_i ↪ h_i \pushout_g g' ↪ (h_i \pushout_g g') \pushout_{g'} g'')(x_{h_i}), λ^{h_i \pushout_g g'}\Big]_{g''}}
    \end{multline*} 
    so $T(X)(g ↪ g' ↪ g'') = T(X)(g ↪ g') \then T(X)(g' ↪ g'')$.
\end{proof}



\subsection{Monad structure}

$T$ can be endowed with the structure of a $\Psh{\BiG\op}$-enriched monad, that is, since $\Psh{\BiG\op}$ is a (cartesian) monoidal closed category, a strong monad. Its unit $η_X：1 → TX^X$ and bind $(-)^\ast：TY^X → TY^{TX}$ are described in the following section.

    Recall that, in the category $\Psh{\BiG\op} ≝ [\BiG, \Sets]$ of covariant presheaves over $\BiG$, the exponential object $Y^X$ is given by $g ↦ [X × \yon(g), Y]$, where 
    \begin{itemize}
        \item $\yon：\BiG\op → [\BiG, \Sets]$ is the covariant Yoneda embedding.
        \item $[X', Y'] = \Nat{X', Y'}$ is the set of natural transformations between two presheaves $X'$ and $Y'$.
    \end{itemize}

\subsubsection{Enriched Bind and Unit} 

\paragraph*{Enriched unit $η_X：1 → TX^X$}:

$$
η_X(g)：
\begin{cases}
    \{*\} &⟶ [X × よ(g), TX]\\
    * &⟼  ŋg'： \begin{cases}
    X(g') × よ(g)(g') &⟶ TX(g') \\
    x_{g'}, \; \text{\textunderscore} &⟼ \Big([0, 1]^{g'_L} ∋ λ ↦ 1 ⋅ \Ket{[x_{g'}, !]_{g'}}\Big)
    \end{cases} 
\end{cases}
$$

\paragraph*{Enriched bind $(-)^\ast：TY^X → TY^{TX}$}:


\begin{gather*} 
    (-)^\ast_g：
    \begin{cases}
    TY^X(g) ⟶ \big[TX × よ(g), \; TY\big]
    \hphantom{\Big(\Prfin \int^{g' ↪ h} X(h)\times [0, 1]^{(h-g')_L}\Big)^{[0,1]^{g_L'}} \!\!\!\!\!\!\!× よ(g)(g') \xto {φ^\ast_{g'}} \Big(\Prfin \int^{g' ↪ h'} Y(h')\times [0, 1]^{(h'-g')_L}\Big)^{[0,1]^{g_L'}}}
    \span\\
    φ ⟼ φ^\ast
    \end{cases}\\    
\text{where } \\[.8em]
φ^\ast_{g'}：\begin{cases}
    \displaystyle\Big(\Prfin \int^{g' ↪ h} \mkern-35mu X(h)\times [0, 1]^{(h-g')_L}\Big)^{[0,1]^{g_L'}} \mkern-15mu × よ(g)(g') \xto {φ^\ast_{g'}} \Big(\Prfin \int^{g' ↪ h'} \mkern-35mu Y(h')\times [0, 1]^{(h'-g')_L}\Big)^{[0,1]^{g_L'}}
    \span\\
    (ϑ, \; g \xinjto {ι} g') \xmapsto {φ^\ast_{g'}} λ' ↦& \letin {ϑ(λ')} {\Braket {\vec p | [x_h, λ^h]_{g'}}_{h ∈ H_{g'}}}{\\
    &\for{h ∈ H_{g'}}\\
    & \;\; \letin{φ_h(x_h, g \xinjto {ι} g' ↪ h)(λ^h ⨆ λ')}{\Braket {\vec {q_h} | [y_h', γ^{h'}]_{h}}_{h' ∈ H_{h}}}{\\
    & \Braket {\vec p | Q | [y_{h'}, γ^{h'} ⨆ λ^h]_{g'}}_{h' ∈ \bigcup\limits_{h ∈ H_{g'}} \mkern-15mu H_h}}}\\
\end{cases}\\
\text{and } \\[.8em]
Q \,≝\, 
    \begin{pmatrix}
        \vec {q_{h_1}} \\
        \vdots \\
        \vec {q_{h_n}}
    \end{pmatrix}_{h_i ∈ H_{g'}}
    =
    \begin{pmatrix}
    q_{h_1, h_1'}   & \rvline &   & \rvline &  q_{h_1, h_m'} \\
    \vdots          & \rvline & ⋯ & \rvline & \vdots \\
    q_{h_n, h_1'}   & \rvline &   & \rvline &  q_{h_n, h_m'}
    \end{pmatrix}_{\substack{h_i ∈ H_{g'} \\ h_j' ∈ \bigcup\limits_{h ∈ H_{g'}} \mkern-15mu H_h}}
\end{gather*}

    In the definition of $Q$, we assume that each $\vec {q_h}$ (for $h ∈ H_{g'}$) has been $0$-padded accordingly.

Internal composition $Z^Y × Y^X \xto {\circ} Z^X$ in the category of presheaves is given by:
        $$∀g, 
        \begin{cases}
        [Y × \yon(g), Z] × [X × \yon(g), Y] &⟶ [X × \yon(g), Z]  \\
        ψ, φ ⟼ X × \yon(g) \xto {1 × Δ} X × \yon(g) × \yon(g) \xto {φ × 1} Y × \yon(g) \xto {ψ} Z\span\\ 
        \end{cases}
        $$
    where $Δ$ is the diagonal functor. 
    In particular, $Z^Y × Y \xto {\ev{} \,=\, \circ} Z$ reduces to: 
    $$
    ∀g, \begin{cases}
    [Y × \yon(g), Z] × Y(g) &⟶ Z(g) \\
    ψ, y &⟼ ψ_g((y, \id_g)) 
    \end{cases}
    $$

    Morphisms $f：X → TY$ in $[\BiG, \Sets]$ will sometimes, by abuse of notation, be identified with their exponential transpose $λ_X. f：1 → TY^X$. Moreover: 
    \begin{equation*}
        f^\ast ≝ 1 \xto f TY^X \xto {(-)^\ast} TY^{TX}
    \end{equation*}

\subsubsection{Associativity and unit laws}

% \begin{align*}
%     f^\ast \circ η = f && η^\ast = \id  \\
%     g^\ast \circ f^\ast = (g^\ast \circ f)^\ast \\
% \end{align*}

\paragraph*{Right unit law $Φ^\ast \circ η = Φ$:} Let us show that
\begingroup
\allowdisplaybreaks
% https://q.uiver.app/?q=WzAsMTUsWzAsMCwiMSJdLFsxLDAsIlRZXlgiXSxbMiwwLCJUWV57VFh9Il0sWzAsMiwiMSJdLFsyLDIsIlRYXlgiXSxbNCwwXSxbNCwxLCJUWV5YIl0sWzUsMF0sWzUsMSwiPSJdLFs2LDBdLFs2LDEsIjEiXSxbNywwXSxbNywxLCJUWV5YIl0sWzAsMSwiw5ciXSxbMiwxLCLDlyJdLFswLDEsIs6mIl0sWzEsMiwiKC0pXlxcYXN0Il0sWzMsNCwizrciLDJdLFsxMCwxMiwizqYiXSxbMTQsNiwiXFxjaXJjIl1d
\begin{tikzcd}
	1 & {TY^X} & {TY^{TX}} && {} & {} & {} & {} \\[-5mm]
	{×} && {×} && {TY^X} & {=} & 1 & {TY^X} \\[-5mm]
	1 && {TX^X}
	\arrow["{Φ}", from=1-1, to=1-2]
	\arrow["{(-)^\ast}", from=1-2, to=1-3]
	\arrow["{η}"', from=3-1, to=3-3]
	\arrow["{Φ}", from=2-7, to=2-8]
	\arrow["\circ", from=2-3, to=2-5]
\end{tikzcd}

First:

\[
Φ^\ast_g = \begin{cases}
    1(g) \xto {Φ_g} [X × \yon(g), TY] \xto {(-)^\ast_g} TY^{TX}(g) \span\\
    \ast ⟼ φ &⟼ (ϑ, g \xinjto {ι} g')\\ 
    &\xmapsto {φ^\ast_{g'}} λ' ↦ \letin{ϑ(λ')}{\Braket {\vec p | [x_h, λ^h]_{g'}}_h}{\\
    & \quad \for{h}\\
        &\quad \qquad \letin{φ_h(x_h, g \xinjto {ι} g' ↪ h)(λ^h ⨆ λ')}{\Braket {\vec {q_h} | [y_{h'}, γ^{h'}]_{h}}_{h'}}{\\
    & \quad \Braket {\vec p | Q | [y_{h'}, γ^{h'} ⨆ λ^h]_{g'}}_{h'}}}
\end{cases}
\]

and 

\[
Φ^\ast_g \,\circ\, η_g = 
\begin{cases}
    (1 × 1) (g) \xto{Φ^\ast_g × η_g} TY^{TX}(g) × TX^X(g) \xto {\circ} TY^X(g) \\
    (\ast, \ast) ⟼ φ^\ast_{g'}, \, ŋ_{g'}\mkern-15mu ⟼ (1 × Δ) \then (ŋ × 1) \then φ^\ast \overset{?}{=} φ
\end{cases}
\]

where

\[
    ŋ_{g'}：\begin{cases}
    X(g') × \yon(g)(g') ⟶ TX(g') \\
    x_{g'}, \; \text{\textunderscore} ⟼ \Bigl([0, 1]^{g_L'} ∋ λ ↦ 1 ⋅ \Ket{[x_{g'}, !]_{g'}} \Bigr)
    \end{cases}
\]

The morphism $X × \yon(g) \xto {1 × Δ} X × \yon(g) × \yon(g) \xto {ŋ × 1} TX × \yon(g) \xto {φ^\ast} TY$ is then given by: 

\[ 
    \begin{cases}
    X(g') × \yon(g)(g') \xto {(\id × Δ)_{g'}} X(g') × \yon(g)(g')^2 \xto {(ŋ × \id)_{g'}} TX(g') × \yon(g)(g') \xto {φ^\ast_ {g'}} TY(g') \span\\
    x_{g'}, \; g \xinjto {ι} g' ⟼  x_{g'}, \; ι, \, ι 
    &⟼ [0, 1]^{g_L'} ∋ λ ↦ 1 ⋅ \Ket{[x_{g'}, !]}, \, ι\\
    &⟼ λ' ↦ \letin{φ_{g'}(x_{g'}, ι)(λ')}{\Braket {\vec q | [y_{h'}, γ^{h'}]_{g'}}_{h'}}{\\
    & \qquad \Braket{1 | \vec q | [y_{h'}, \smash{\underbrace{γ^{h'} \, ⨆ \, !}_{\mathclap{= \, γ^{h'}}}}]_{g'}}_{h'}}
    \end{cases}    
\]

\paragraph*{Left unit law $η^\ast = \id$:} Let us show that

$$1 \xto {η} TX^X \xto {(-)^\ast} TX^{TX} = 1 \xto {λ_{TX}. \,\id} TX^{TX}$$

The left-hand side (LHS) is equal to:

\begin{alignat*}{2}
    \ast &\xmapsto {η_g} ŋ_{g'}：
    \begin{cases}
        X(g') × \yon(g)(g') ⟶ TX(g')\\
        x_{g'}, \; \text{\textunderscore} ⟼ \Bigl([0, 1]^{g_L'} ∋ λ ↦ 1 ⋅ \Ket{[x_{g'}, !]} \Bigr)\\
    \end{cases} \span\span\\
    &\xmapsto {(-)^\ast g} ϑ, g \xinjto {ι} g' \xmapsto{ŋ^\ast_{g'}} λ' ⟼ 
    &&\;\;\letin{ϑ(λ')}{\Braket {\vec p | [x_h, λ^h]_{g'}}_h}{\\
    & &&\;\;\for{h} \letin{ŋ_h(x_h, \, g \xinjto {ι} g' ↪ h)(λ^h ⨆ λ')}{1 ⋅ \Ket{[x_h, !]_h}}{\\ 
    & &&\;\;\Braket{\vec p | \smash{\underbrace{\mathbf I}_{\mathclap{\text{\small identity matrix}}}} | [x_h, \, \smash{\underbrace{! \,⨆\, λ^h}_{= \, λ^h}}]_{g'}}_h}}\\
    & && \qquad \qquad \qquad \qquad \qquad \qquad \; \raisebox{-1.7em}{\verteq}\\[-.2cm]
    & && \qquad \qquad \qquad \qquad \underbrace{ϑ, \, ι \xmapsto {ŋ^\ast_{g'}} λ' ⟼ ϑ(λ')}_{= \, \text{RHS}}
\end{alignat*}

\paragraph*{Associativity $Ψ^\ast \circ Φ^\ast = (Ψ^\ast \circ Φ)^\ast$:} Let us show that

% https://q.uiver.app/?q=WzAsMjIsWzAsMCwiMSJdLFsxLDAsIlRaXlkiXSxbMiwwLCJUWl57VFl9Il0sWzAsMiwiMSJdLFsxLDIsIlRZXlgiXSxbNCwwXSxbMywxLCJUWV57VFh9Il0sWzAsNCwiMSJdLFsxLDMsIlxcVmVydCJdLFsxLDQsIlRaXlkiXSxbMiw0LCJUWl57VFl9Il0sWzAsMSwiw5ciXSxbMiwxLCLDlyJdLFsyLDIsIlRZXntUWH0iXSxbMSwxLCLDlyJdLFswLDUsIsOXIl0sWzAsNiwiMSJdLFs2LDNdLFsyLDYsIlRZXlgiXSxbMiw1LCLDlyJdLFszLDUsIlRZXlgiXSxbNCw1LCJUWV57VFh9Il0sWzAsMSwizqgiXSxbMSwyLCIoLSleXFxhc3QiXSxbMyw0LCLOpiIsMl0sWzEyLDYsIlxcY2lyYyJdLFs3LDksIs6oIl0sWzksMTAsIigtKV5cXGFzdCJdLFsxNiwxOCwizqYiLDJdLFsyMCwyMSwiKC0pXlxcYXN0Il0sWzQsMTMsIigtKV5cXGFzdCIsMl0sWzE5LDIwLCJcXGNpcmMiXV0=
\[\begin{tikzcd}
	1 & {TZ^Y} & {TZ^{TY}} && {} \\
	{×} & {×} & {×} & {TY^{TX}} \\
	1 & {TY^X} & {TY^{TX}} \\
	& \Vert &&&&& {} \\
	1 & {TZ^Y} & {TZ^{TY}} \\
	{×} && {×} & {TY^X} & {TY^{TX}} \\
	1 && {TY^X}
	\arrow["{Ψ}", from=1-1, to=1-2]
	\arrow["{(-)^\ast}", from=1-2, to=1-3]
	\arrow["{Φ}"', from=3-1, to=3-2]
	\arrow["\circ", from=2-3, to=2-4]
	\arrow["{Ψ}", from=5-1, to=5-2]
	\arrow["{(-)^\ast}", from=5-2, to=5-3]
	\arrow["{Φ}"', from=7-1, to=7-3]
	\arrow["{(-)^\ast}", from=6-4, to=6-5]
	\arrow["{(-)^\ast}"', from=3-2, to=3-3]
	\arrow["\circ", from=6-3, to=6-4]
\end{tikzcd}\]

The LHS

$$(Ψ^\ast_g × Φ^\ast_g) \then \circ = (1(g) × 1(g) \xto {Ψ_g × Φ_g} TZ^Y(g) × TY^{TX}(g) \xto {(-)^\ast_g × (-)^\ast_g} TZ^{TY}(g) × TY^{TX}(g)) \then \circ$$

is equal to:


\begin{alignat*}{3}
& \ast, \ast  ⟼ \, \substack{\textstyle ψ ∈ [Y × \yon(g), TZ], \\ \textstyle φ ∈ [X × \yon(g), TY]} \, \span\span \\
& ⟼ \; 
&& \bigg(ϑ, g \xinjto {ι} g' \xmapsto {ψ^\ast_{g'}} λ' ↦ && \; \letin{ϑ(λ')}{\Braket{\vec r | [y_h, θ^h]_{g'}}_h}{ \\
&    && &&\; \for{h} \\
&    && &&\; \quad \letin{ψ(y_h, \; g \xinjto {ι} g' ↪ h)(θ^h ⨆ θ')}{\Braket{\vec {s_h} | [z_{h'}, χ^{h'}]_h}_{h'}}{\\
&    && &&\; \Braket{\vec r | S | \vphantom{θ^h}\smash{[z_{h'}, \, χ^{h'} \,⨆\, θ^h]_{g'}}}_{h'}}}\bigg),\\
&   && \bigg(ϑ, g \xinjto {ι} g' \xmapsto {φ^\ast_{g'}} λ' ↦ &&\; \letin{ϑ(λ')}{\Braket{\vec p | [x_h, λ^h]_{g'}}_{h'}}{ \\
&    && &&\; \for{h} \\ 
&    && &&\; \quad \letin{φ(x_h, \; g \xinjto {ι} g' ↪ h)(λ^h ⨆ λ')}{\Braket{\vec {q_h} | [y_{h'}, γ^{h'}]_h}_{h'}}{\\
&    && &&\; \Braket{\vec p | Q | \vphantom{θ^h}\smash{[y_{h'}, \, γ^{h'} \,⨆\, λ^h]_{g'}}}_{h'}}}\bigg)\\
&  &&  \hspace{-2.5em} \overset{\circ}{⟼} \; \underbrace{(1 × Δ) \then (φ^\ast × 1) \then ψ^\ast}_{= \, α} \overset{?}{=} \underbrace{((1 × Δ) \then (φ × 1) \then ψ^\ast)^\ast}_{= \, \text{RHS} \, ≝ \, β} \span \span
\end{alignat*}

where the map $$α \,≝\, TX × \yon(g) \xto {1 × Δ} TX × \yon(g)^2 \xto {φ^\ast × 1} TY × \yon(g) \xto {ψ^\ast} TZ$$ 

is given by

\begin{alignat*}{3}
&TX(g') × \yon(g)(g') \xto {(1 × Δ)_{g'}} TX(g') × \yon(g)(g')^2 \xto {φ^\ast_{g'} \,×\, \id_{g'}} TY(g') × \yon(g)(g') \xto {ψ^\ast_{g'}} TZ(g') \span\span \span\span  \\
&ϑ, ι &&↦ ϑ, \, ι, ι ↦ \Big(λ' \xmapsto {φ^\ast_{g'}(ϑ, ι)} &&\; \letin{ϑ(λ')}{\Braket{\vec p | [x_h, λ^h]_{g'}}_h}{ \\
& && && \; \for{h} \; \\
& && && \; \quad \letin{φ_h(x_h, \; g \xinjto {ι} g' ↪ h)(λ^h ⨆ λ')}{\Braket{\vec {q_h} | [y_{h'}, γ^{h'}]_h}_{h'}}{\\
& && && \quad \Braket{\vec p | Q | \vphantom{θ^h}\smash{[y_{h'}, \, γ^{h'} \,⨆\, λ^h]_{g'}}}_{h'}}}\Big), \; ι\\
& && \xmapsto {ψ^\ast_{g'}} λ' ↦ &&\hspace{-4.5em} \letin{φ^\ast_{g'}(ϑ, ι)(λ')}{\Braket{\vec p | Q | [y_{h'}, γ^{h'} \,⨆\, λ^h]_{g'}}_{h'}}{ \\
& && && \hspace{-4.5em} \for{h'} \; \\
& && && \hspace{-3.5em} \letin{ψ_{h'}(y_{h'}, \; g \xinjto {ι} g' ↪ h')(γ^{h'} \,⨆\, λ^h ⨆ λ')}{\Braket{\vec {s_{h'}} | [z_{h''}, χ^{h''}]_{h'}}_{h''}}{\\
& && && \hspace{-4.5em} \Braket{\vec p | Q | S | \vphantom{θ^h}\smash{[z_{h''}, \, χ^{h''} \,⨆\, γ^{h'} \,⨆\, λ^h]_{g'}}}_{h''}}}\\
& && \verteq \span\span \\
&ϑ, ι &&↦ ϑ, \, ι, ι ↦ λ' \xmapsto {φ^\ast_{g'}(ϑ, ι)} &&\; \letin{ϑ(λ')}{\Braket{\vec p | [x_h, λ^h]_{g'}}_h}{ \\
& && && \; \for{h} \; \\
& && && \quad \letin{φ_h(x_h, \; g \xinjto {ι} g' ↪ h)(λ^h ⨆ λ')}{\Braket{\vec {q_h} | [y_{h'}, γ^{h'}]_h}_{h'}}{\\
& && && \; \for{h'} \; \\
& && && \quad \letin{ψ_{h'}(y_{h'}, \; g \xinjto {ι} g' ↪ h')(γ^{h'} \,⨆\, λ^h ⨆ λ')}{\\
& && && \quad \hspace{14.3em}\Braket{\vec {s_{h'}} | [z_{h''}, χ^{h''}]_{h'}}_{h''}}{\\
& && && \; \Braket{\vec p | Q | S | \vphantom{θ^h}\smash{[z_{h''}, \, χ^{h''} \,⨆\, γ^{h'} \,⨆\, λ^h]_{g'}}}_{h''}}}}\\
\end{alignat*}

As for the map $$β \,≝\, (X × \yon(g) \xto {1 × Δ} X × \yon(g) × \yon(g) \xto {φ × 1} TY × \yon(g) \xto {ψ^\ast} TZ)^\ast$$
we have 
\begin{alignat*}{3}
    &X(g') × \yon(g)(g') \xto {\id_{g'} × Δ_{g'}} X(g') × \yon(g)(g')^2 \xto {φ_{g'} \,×\, \id_{g'}} TY(g') × \yon(g)(g') \xto {ψ^\ast_{g'}} TZ(g') \span\span \span\span \\
    &x_{g'}, \, g \xinjto{ι} g' &&⟼ x_{g'}, \, ι, ι \span\span\\
    & &&⟼ φ_{g'}(x_{g'}, ι), \, ι \span\span\\
    & &&\xmapsto{ψ^\ast_{g'}} λ' ↦ &&\; \letin{φ_{g'}(x_{g'}, ι)(λ')}{\Braket{\vec q | [y_{h'}, γ^{h'}]_{g'}}_{h'}}{ \\
    & && && \; \for{h'} \; \\
    & && && \; \quad \letin{ψ_{h'}(y_{h'}, \; g \xinjto {ι} g' ↪ h')(γ^{h'} \,⨆\, λ')}{\Braket{\vec {s_{h'}} | [z_{h''}, χ^{h''}]_{h'}}_{h''}}{\\
    & && && \; \Braket{\vec q | S | \vphantom{θ^h}\smash{[z_{h''}, \, χ^{h''} \,⨆\, γ^{h'}]_{g'}}}_{h''}}}
\end{alignat*}

So that $β$ is given by:
\begin{alignat*}{3}
    &TX(g') × \yon(g)(g') \xto {ζ^\ast(g') 
    \,≝\, \big((\id(g') × Δ(g')) \,\then\, (φ(g') × \id(g')) \,\then\, ψ^\ast(g')\big)^\ast} TZ(g') \span\span\\
    & ϑ, \, ι ⟼ λ' ⟼ && \;\letin{ϑ(λ')}{\Braket{\vec p | [x_h, λ^h]_{g'}}_h}{ \\
    & && \; \for{h} \; \\
    & && \; \quad \letin{ζ_h(x_h, \; g \xinjto {ι} g' ↪ h)(λ^h ⨆ λ')}{\\
    & && \; \quad \hspace{10em}\Braket{\vec {q_h} | S_h | \vphantom{θ^h}\smash{[z_{h''}, \, χ^{h''} \,⨆\, γ^{h'} \,⨆\, λ^h]_{g'}}}_{h''}}{ \\
    & && \; \Braket{\vec p | Q | S | \vphantom{θ^h}\smash{[z_{h''}, \, χ^{h''} \,⨆\, γ^{h'} \,⨆\, λ^h]_{g'}}}_{h''}}}\\
    & && \verteq \\
    & ϑ, \, ι ⟼  λ' ⟼ && \;\letin{ϑ(λ')}{\Braket{\vec p | [x_h, λ^h]_{g'}}_h}{ \\
    & && \; \for{h} \\
    & && \; \;\; \letin{φ(x_h, \; g \xinjto {ι} g' ↪ h)(λ^h ⨆ λ')}{\Braket{\vec {q_h} | [y_{h'}, γ^{h'}]_{h}}_{h'}}}{ \\
    & && \; \quad \for{h'} \\
    & && \; \quad \;\; \letin{ψ_{h'}(y_{h'}, \; g \xinjto {ι} g' ↪ h')(γ^{h'} \,⨆\, λ^h \,⨆\, λ')}{\Braket{\vec {s_{h'}} | [z_{h''}, χ^{h''}]_{h'}}_{h''}}{\\
    % & && \; \qquad \Braket{\vec {q_h} | S_h | \vphantom{θ^h}\smash{[z_{h''}, \, χ^{h''} \,⨆\, γ^{h'} \,⨆\, λ^h]_{g'}}}_{h''}} \\
    & && \; \Braket{\vec p | Q | S | \vphantom{θ^h}\smash{[z_{h''}, \, χ^{h''} \,⨆\, γ^{h'} \,⨆\, λ^h]_{g'}}}_{h''}}}
\end{alignat*}
\endgroup

Therefore, $α = β$.

\subsection{Strong commutativity}

\begin{theorem}[Strong commutativity]
    $T$ is a strong commutative monad, \ie in the internal language of the topos: for every $a：1 → TA, b：1 → TB$:
    \begin{equation}\label{eq:strongcomm}
        a \bind \lambdaabs{x}{b \bind \lambdaabs{y}{η(x, y)}} \;=\; b \bind \lambdaabs{y}{a \bind \lambdaabs{x}{η(x, y)}}
    \end{equation}
\end{theorem}

\begin{proof}
\begingroup
\allowdisplaybreaks
The term $b \bind \lambdaabs{y}{η(x, y)}$ is given by:

% https://q.uiver.app/?q=WzAsOCxbMCwwLCJBIl0sWzEsMCwiVChBw5dCKV5CIl0sWzIsMCwiVChBw5dCKV57VEJ9Il0sWzAsMSwiw5ciXSxbMCwyLCIxIl0sWzIsMiwiVEIiXSxbMiwxLCLDlyJdLFszLDEsIlQoQcOXQikiXSxbMCwxLCLOu19CLiDOtyJdLFsxLDIsIigtKV5cXGFzdCJdLFs0LDUsImIiLDJdLFs2LDcsIntcXHJtIGV2fSJdXQ==
\[\begin{tikzcd}
	A & {T(A×B)^B} & {T(A×B)^{TB}} \\[-5mm]
	{×} && {×} & {T(A×B)} \\[-5mm]
	1 && TB
	\arrow["{λ_B. η}", from=1-1, to=1-2]
	\arrow["{(-)^\ast}", from=1-2, to=1-3]
	\arrow["b"', from=3-1, to=3-3]
	\arrow["{{\rm ev}}", from=2-3, to=2-4]
\end{tikzcd}\]

So \cref{eq:strongcomm} corresponds to the following equality of commutative diagrams:

% https://q.uiver.app/?q=WzAsMTcsWzAsMCwiMSJdLFswLDIsIjEiXSxbMCwxLCLDlyJdLFszLDAsIlQoQcOXQileQSJdLFs0LDAsIlQoQcOXQilee1RBfSJdLFs0LDIsIlRBIl0sWzQsMSwiw5ciXSxbNSwxLCJUKEHDl0IpIl0sWzMsMywiXFx2ZXJ0ZXEiXSxbMCw0LCIxIl0sWzMsNCwiVChBw5dCKV5CIl0sWzQsNCwiVChBw5dCKV57VEJ9Il0sWzAsNiwiMSJdLFs0LDYsIlRCIl0sWzAsNSwiw5ciXSxbNCw1LCLDlyJdLFs1LDUsIlQoQcOXQikiXSxbMCwzLCLOu19BLiBcXEJpZyhcXGJpZygozrtfQi4gzrcpXlxcYXN0IMOXIGJcXGJpZykgXFx0aGVuIHtcXHJtIGV2fVxcQmlnKSJdLFszLDQsIigtKV5cXGFzdCJdLFsxLDUsImEiLDJdLFs2LDcsIntcXHJtIGV2fSJdLFs5LDEwLCLOu19CLiBcXEJpZyhcXGJpZygozrtfQS4gzrcpXlxcYXN0IMOXIGFcXGJpZykgXFx0aGVuIHtcXHJtIGV2fVxcQmlnKSJdLFsxMCwxMSwiKC0pXlxcYXN0Il0sWzEyLDEzLCJiIiwyXSxbMTUsMTYsIntcXHJtIGV2fSJdXQ==
\[\begin{tikzcd}
	1 &&& {T(A×B)^A} & {T(A×B)^{TA}} \\[-5mm]
	{×} &&&& {×} & {T(A×B)} \\[-5mm]
	1 &&&& TA \\
	&&& \verteq \\
	1 &&& {T(A×B)^B} & {T(A×B)^{TB}} \\[-5mm]
	{×} &&&& {×} & {T(A×B)} \\[-5mm]
	1 &&&& TB
	\arrow["{λ_A. \Big(\big((λ_B. η)^\ast × b\big) \,\then\, {\rm ev}\Big)}", from=1-1, to=1-4]
	\arrow["{(-)^\ast}", from=1-4, to=1-5]
	\arrow["a"', from=3-1, to=3-5]
	\arrow["{{\rm ev}}", from=2-5, to=2-6]
	\arrow["{λ_B. \Big(\big((λ_A. η)^\ast × a\big) \,\then\, {\rm ev}\Big)}", from=5-1, to=5-4]
	\arrow["{(-)^\ast}", from=5-4, to=5-5]
	\arrow["b"', from=7-1, to=7-5]
	\arrow["{{\rm ev}}", from=6-5, to=6-6]
\end{tikzcd}\]

Step by step, this unfolds as:

\begin{itemize}
\item $A \xto {λ_B. η} T(A × B)^B$:
\begin{align*}
    &A(g) \xto {(λ_B. η)_g} T(A × B)^B(g)\\
    & x ⟼ ŋ_{g'}^x： \begin{cases}
    B(g') × \yon(g, g') ⟶ T(A × B)(g')\\
    y, \, g \xinjto {ι} g' ⟼ \Big(λ' ↦ 1 ⋅ \Ket{\big[(A(ι)(x), y), !\big]_{g'}}\Big)
    \end{cases}
\end{align*}

\item $A \xto {λ_B. η} T(A × B)^B \xto {(-)^\ast} T(A × B)^{TB}$:
\begin{alignat*}{2}
    &A(g) \xto {(λ_B. η)_g} [B × \yon(g), \, T(A × B)] \xto {(-)^\ast_g} [TB × \yon(g),\, T(A × B)]\span\span\\
    &x ↦ ŋ^x ↦ (ϑ, g \xinjto{ι} g') \xmapsto{{ŋ^x}^\ast_{g'}} λ' \,↦\, &&\letin{ϑ(λ')}{\Braket {\vec q | [y_h,\, γ^h]_{g'}}_h}{ \\
    & && \for{h}\\
    & && \quad \; \letin{ŋ^x_h(y_h,\, g \xinjto {ι} g' ↪ h)(γ^h ⨆ λ')}{\\
    & && \quad \; \;\;\; 1 ⋅ \Ket{\big[(A(g \xinjto {ι} g' ↪ h)(x), y_h),\, !\big]_h}}\\
    & && \Braket{\vec q | \smash{\underbrace{\mathbf{I}}_{\mathclap{\text{\small each line is a one-hot vector}}}} | \big[(A(g \xinjto {ι} g' ↪ h)(x), y_h), γ^h\big]_{g'}}_h}
\end{alignat*}\\
\item $% https://q.uiver.app/?q=WzAsOCxbMCwwLCJBIl0sWzEsMCwiVChBIMOXIEIpXkIiXSxbMiwwLCJUKEHDl0IpXntUQn0iXSxbMCwyLCIxIl0sWzIsMiwiVEIiXSxbMCwxLCLDlyJdLFsyLDEsIsOXIl0sWzMsMSwiVChBIMOXIEIpIl0sWzAsMSwizrtfQi4gzrciXSxbMSwyLCIoLSleXFxhc3QiXSxbMyw0LCJiIiwyXSxbNiw3LCJ7XFxybSBldn0iXV0=
\begin{tikzcd}
	A & {T(A × B)^B} & {T(A×B)^{TB}} \\[-8mm]
	{×} && {×} & {T(A × B)} \\[-8mm]
	1 && TB
	\arrow["{λ_B. η}", from=1-1, to=1-2]
	\arrow["{(-)^\ast}", from=1-2, to=1-3]
	\arrow["b"', from=3-1, to=3-3]
	\arrow["{{\rm ev}}", from=2-3, to=2-4]
\end{tikzcd}$:
\begin{alignat*}{3}
    &A(g) × 1(g) \xto {(λ_B. η)^\ast_g × b_g} [TB × \yon(g), \, T(A × B)] × TB(g) \xto {\ev{}} T(A × B)(g)\span\span \span\span\\
    &x, \ast &&↦ \Big(ϑ, g \xinjto{ι} g' \xmapsto{{ŋ^x}^\ast_{g'}} λ' \,↦\, && \; \letin{ϑ(λ')}{\Braket {\vec q | [y_h,\, γ^h]_{g'}}_h}{ \\
    & && && \; \for{h}\\
    & && && \quad \; \letin{ŋ^x_h(y_h,\, g \xinjto {ι} g' ↪ h)(γ^h ⨆ λ')}{\\
    & && && \quad \; \;\;\; 1 ⋅ \Ket{\big[(A(g \xinjto {ι} g' ↪ h)(x), y_h),\, !\big]_h}}\\
    & && && \Braket{\vec q | \big[(A(g \xinjto {ι} g' ↪ h)(x), y_h), γ^h\big]_{g'}}_h}\Big), b_g(\ast)\\
    & && ↦ λ \xmapsto{{ŋ^x}^\ast_g(b_g(\ast),\, \id_g)} &&\mkern-35mu \letin{b_g(\ast)(λ)}{\Braket {\vec q | [y_h,\, γ^h]_{g'}}_h}{ \\
    & && && \mkern-35mu \for{h} \; \letin{ŋ^x_h(y_h,\, g ↪ h)(γ^h ⨆ λ)}{\\
    & && && \mkern-35mu \hphantom{\for{h} \;}\;\;\; 1 ⋅ \Ket{\big[(A(g ↪ h)(x), y_h),\, !\big]_h}} \\
    & && && \mkern-35mu \Braket{\vec q | \big[(A(g ↪ h)(x), y_h), γ^h\big]_g}_h}
\end{alignat*}\\
\item $1 \xto {λ_A. \Big(\big((λ_B. η)^\ast × b\big) \,\then\, \ev{}\Big)} T(A × B)^A$:
\begin{alignat*}{2}
    &1(g) ⟶ T(A × B)^A(g) \span\span\\
    &\ast ⟼ φ_{g'}： \begin{cases}
    A(g') × \yon(g)(g') ⟶ T(A×B(g')\\
    x, \, \text{\textunderscore} ⟼ λ \xmapsto{{ŋ^x}^\ast_g} \; \letin{b_g(\ast)(λ)}{\Braket {\vec q | [y_h,\, γ^h]_g}_h}{ \\
    \hspace{7.2em} \for{h} \; \letin{ŋ^x_h(y_h,\, g ↪ h)(γ^h ⨆ λ)}{\\
    \hspace{8em} \hphantom{\for{h} \;} 1 ⋅ \Ket{\big[(A(g ↪ h)(x), y_h),\, !\big]_h}} \\
    \hspace{7.2em} \Braket{\vec q | \big[(A(g ↪ h)(x), y_h), γ^h\big]_g}_h}
    \end{cases}
\end{alignat*}
\item $1 \xto {λ_A. \Big(\big((λ_B. η)^\ast × b\big) \,\then\, \ev{}\Big)} T(A × B)^A \xto {(-)^\ast} T(A × B)^{TA}$:
\begin{alignat*}{2}
    &1(g) \xto {λ_A. \Big(\big((λ_B. η)^\ast × b\big) \,\then\, \ev{}\Big)_g} T(A × B)^A(g) \xto {(-)^\ast_g} T(A × B)^{TA}(g)\span\span \\
    &\ast ↦ φ ↦ (ϑ, g \xinjto{ι} g') \xmapsto{φ^\ast_{g'}} λ' \,↦\, && \; \letin{ϑ(λ')}{\Braket {\vec p | [x_h,\, λ^h]_{g'}}_h}{ \\
    & && \; \for{h} \; \\
    & &&  \; \quad \letin{φ_h(x_h,\, g \xinjto {ι} g' ↪ h)(λ^h ⨆ λ')}{\\
    & &&  \; \quad \qquad \Braket{\vec {q_h} | \big[(A(h ↪ h')(x_h), γ^{h'}\big]_h}_{h'}}{\\
    & && \; \Braket{\vec p | Q | \big[(A(h ↪ h')(x_h), y_{h'}), γ^{h'} \,⨆\, λ^h \big]_{g'}}_{h'}}}\\
\end{alignat*}
\item $% https://q.uiver.app/?q=WzAsOSxbMCwwLCIxIl0sWzMsMCwiVChBw5dCKV5BIl0sWzUsMCwiVChBw5dCKV57VEF9Il0sWzAsMSwiw5ciXSxbMCwyLCIxIl0sWzUsMiwiVEEiXSxbNSwxLCLDlyJdLFs2LDEsIlQoQcOXQikiXSxbMiwwXSxbMCwxLCLOu19BLiBcXEJpZyhcXGJpZygozrtfQi4gzrcpXlxcYXN0IMOXIGJcXGJpZykgXFx0aGVuIHtcXHJtIGV2fVxcQmlnKSJdLFsxLDIsIigtKV5cXGFzdCJdLFs0LDUsImEiLDJdLFs2LDcsIntcXHJtIGV2fSJdXQ==
\begin{tikzcd}
	1 && {} & {T(A×B)^A} && {T(A×B)^{TA}} \\[-8mm]
	{×} &&&&& {×} & {T(A×B)} \\[-8mm]
	1 &&&&& TA
	\arrow["{λ_A. \Big(\big((λ_B. η)^\ast × b\big) \,\then\, {\rm ev}\Big)}", from=1-1, to=1-4]
	\arrow["{(-)^\ast}", from=1-4, to=1-6]
	\arrow["a"', from=3-1, to=3-6]
	\arrow["{{\rm ev}}", from=2-6, to=2-7]
\end{tikzcd}$:
\begin{alignat*}{3}
    &(1×1)(g) \xto {\Big(λ_A. \big(\big((λ_B. η)^\ast × b\big) \,\then\, \ev{}\big)_g \,\then\, (-)^\ast_g\Big) \,×\, a_g} T(A × B)^A(g) × TA(g) \xto {\ev{g}} T(A × B)(g)\span\span \span\span\\
    &\ast, \ast &&↦ \Big(ϑ, ι \xmapsto{φ^\ast_{g'}} λ' \,↦\, && \; \letin{ϑ(λ')}{\Braket {\vec p | [x_h,\, λ^h]_{g'}}_h}{ \\
    & && && \; \for{h} \; \\
    & && &&  \; \quad \letin{φ_h(x_h,\, g \xinjto {ι} g' ↪ h)(λ^h ⨆ λ')}{\\
    & && &&  \; \quad \quad \Braket{\vec {q_h} | \big[(A(h ↪ h')(x_h), γ^{h'}\big]_h}_{h'}}{\\
    & && && \; \Braket{\vec p | Q | \big[(A(h ↪ h')(x_h), y_{h'}), γ^{h'} \,⨆\, λ^h \big]_{g'}}_{h'}}} \Big), \; a_g(\ast)\\
    & &&↦ λ \xmapsto{φ^\ast_g(a_g(\ast),\, \id_g)}\; &&  \letin{a_g(\ast)(λ)}{\Braket{\vec p | [x_h,\, λ^h]_g}_h}{\\
    & && &&  \; \qquad \for{h} \; \\
    & && &&  \; \qquad \quad \letin{φ_h(x_h,\, g ↪ h)(λ^h ⨆ λ)}{\\
    & && &&  \; \qquad \quad \qquad \Braket{\vec {q_h} | \big[(A(h ↪ h')(x_h), y_{h'}), γ^{h'} \big]_{h}}_{h'}}{\\
    & && &&  \; \Braket{\vec p | Q | \big[(A(h ↪ h')(x_h), y_{h'}), γ^{h'} \,⨆\, λ^h \big]_g}_{h'}}}\\
    & &&↦ λ \xmapsto{φ^\ast_g(a_g(\ast),\, \id_g)}\; && \letin{a_g(\ast)(λ)}{\Braket{\vec p | [x_h,\, λ^h]_g}_h}{\\
    & && &&  \;\; \for{h} \\
    & && &&  \;\; \;\; \letin{b_h(\ast)(λ^h ⨆ λ)}{\Braket{\vec {q_h} | [y_{h'}, \, γ^{h'}]_h}_{h'}}{\\
    & && &&  \;\; \;\; \;\; \for{h'} \; \\
    & && &&  \;\; \;\; \;\; \;\; \letin{ŋ^{x_h}_{h'}(y_{h'}, h ↪ h')(γ^{h'} ⨆ λ^h ⨆ λ)}{\\
    & && &&  \;\; \;\; \;\; \;\; \;\; \qquad \;\; \;\; 1 ⋅ \Ket{\bigl[(A(h ↪ h')(x_h), y_{h'}), !\bigr]_{h'}}}{\\
    & && &&  \; \Braket{\vec p | Q | \big[(A(h ↪ h')(x_h), y_{h'}), γ^{h'} \,⨆\, λ^h \big]_g}_{h'}}}}
\end{alignat*} 
\end{itemize}

Commutativity then boils down to this last map $φ^\ast_g(a_g(\ast),\, \id_g)$ being equal to:

\begin{align*}
    λ \xmapsto{ψ^\ast_g(b_g(\ast),\, \id_g)}\; & \letin{b_g(\ast)(λ)}{\Braket{\vec q | [y_h,\, γ^h]_g}_h}{\\
    & \;\; \for{h} \\
    & \;\; \;\; \letin{a_h(\ast)(γ^h ⨆ λ)}{\Braket{\vec {p_h} | [x_{h'}, \, λ^{h'}]_h}_{h'}}{\\
    & \;\; \;\; \;\; \for{h'} \; \\
    & \;\; \;\; \;\; \;\; \letin{ŋ^{y_h}_{h'}(x_{h'}, h ↪ h')(λ^{h'} ⨆ γ^h ⨆ λ)}{1 ⋅ \Ket{\bigl[(x_{h'}, B(h ↪ h')(y_h)), !\bigr]_{h'}}}{\\
    & \; \Braket{\vec q | P | \big[(x_{h'}, B(h ↪ h')(y_h)), λ^{h'} \,⨆\, γ^h \big]_g}_{h'}}}}
\end{align*}

And they turn out to be equal indeed: by naturality of $a：1 → TA, \, b：1 → TB$, we have, for every $h_0$ in the coslice category $g/\BiG$:

% https://q.uiver.app/?q=WzAsMyxbMCwxLCJcXGFzdCJdLFsxLDAsImFfZyhcXGFzdCkozrspIOKJnSBcXEJyYWtldHtcXHZlYyBwIHwgW3hfaCxcXCwgzrteaF1fZ31faCAiXSxbMSwyLCJhX3toXzB9KFxcYXN0KSjOs157aF8wfSBcXCziqIZcXCwgzrspIOKJnSBcXEJyYWtldHtcXHZlYyB7cF97aF8wfX0gfCBbeF97aCd9LFxcLCDOu157aCd9XV97aF8wfX1fe2gnfSA9IFxcQnJha2V0e1xcdmVjIHAgfCBbQShoIOKGqiBoXzAgXFxjb3Byb2RfZyBoKSh4X2gpLFxcLCDOu15oXV97aF8wfX1faCAgIl0sWzAsMSwiYV9nIiwwLHsic3R5bGUiOnsidGFpbCI6eyJuYW1lIjoibWFwcyB0byJ9fX1dLFswLDIsImFfe2hfMH0iLDIseyJzdHlsZSI6eyJ0YWlsIjp7Im5hbWUiOiJtYXBzIHRvIn19fV0sWzEsMiwiVEEoZyDihqogaCkiLDAseyJzdHlsZSI6eyJ0YWlsIjp7Im5hbWUiOiJtYXBzIHRvIn19fV1d
\[\begin{tikzcd}
	& {a_g(\ast)(λ) ≝ \Braket{\vec p | [x_h,\, λ^h]_g}_h } \\
	\ast \\
	& {a_{h_0}(\ast)(γ^{h_0} \,⨆\, λ) ≝ \Braket{\vec {p_{h_0}} | [x_{h'},\, λ^{h'}]_{h_0}}_{h'} = \Braket{\vec p | [A(h ↪ h_0 \coprod_g h)(x_h),\, λ^h]_{h_0}}_h  }
	\arrow["{a_g}", maps to, from=2-1, to=1-2]
	\arrow["{a_{h_0}}"', maps to, from=2-1, to=3-2]
	\arrow["{TA(g ↪ h)}", maps to, from=1-2, to=3-2]
\end{tikzcd}\]

and likewise for $b$. The equality $\Braket{\vec {p_{h_0}} | [x_{h'},\, λ^{h'}]_{h_0}}_{h'} = \Braket{\vec p | [A(h ↪ h_0 \coprod_g h)(x_h),\, λ^h]_{h_0}}_h$ implies that $h'$ and $h$ range over the same index set. 

Therefore, if $b_g(\ast)(λ) ≝ \Braket{\vec q | [y_{h'},\, γ^{h'}]_g}_{h'}$, the map $φ^\ast_g(a_g(\ast),\, \id_g)$ can be written as:
\begin{align*}
    λ ↦\; & \letin{a_g(\ast)(λ)}{\Braket{\vec p | [x_h,\, λ^h]_g}_h}{\\
    & \;\; \for{h} \\
    & \;\; \;\; \letin{b_h(\ast)(λ^h ⨆ λ)}{\Braket{\vec q | [B(h' ↪ h \,{\textstyle \pushout}_g\, h')(y_{h'}), \, γ^{h'}]_h}_{h'}}{\\
    &  \;\; \;\; \;\; \for{h'} \; \\
    &  \;\; \;\; \;\; \;\; \letin{ŋ^{x_h}_{h \,{\scriptsize \pushout}_g\, h'}(B(h' ↪ h \,{\textstyle \pushout}_g\, h')(y_{h'}), h ↪ h \,{\textstyle \pushout}_g\, h')(γ^{h'} ⨆ λ^h ⨆ λ)}{\\
    &  \;\; \;\; \;\; \;\; \hspace{10em} 1 ⋅ \Ket{\bigl[(A(h ↪ h \,{\textstyle \pushout}_g\, h')(x_h), B(h' ↪ h \,{\textstyle \pushout}_g\, h')(y_{h'})), !\bigr]_{h'}}}{\\
    &  \; \Braket{\vec p | \mathbf{I} ⊗ {\Bra{\vec q}} | \big[(A(h ↪ h \,{\textstyle \pushout}_g\, h')(x_h), B(h' ↪ h \,{\textstyle \pushout}_g\, h')(y_{h'})), γ^{h'} \,⨆\, λ^h \big]_g}_{h'}}}}
\end{align*}

where $$\mathbf{I} ⊗ {\Bra{\vec q}} ≝ \begin{pmatrix}
    \Bra{\vec q} & & {\raisebox{-1em}[0pt][0pt]{\!\!\!\!\bigzero}} \\
    & \ddots & \\
    {\raisebox{.5em}[0pt][0pt]{\;\;\;\bigzero}} &  & \Bra{\vec q}
\end{pmatrix}$$ is the Kronecker product, so that $\Braket{\vec p} (\mathbf{I} ⊗ {\Bra{\vec q}})$ is the row vector $\big(p_{h_1} ⋅ \Bra{\vec q} \quad ⋯ \quad p_{h_n} ⋅ \Bra{\vec q}\big)$.

Similarly, if $a_g(\ast)(λ) ≝ \Braket{\vec p | [x_h,\, λ^h]_g}_h$, the map $ψ^\ast_g(b_g(\ast),\, \id_g)$ can be written as:

\begin{align*}
    λ ↦\; & \letin{b_g(\ast)(λ)}{\Braket{\vec q | [y_{h'},\, γ^{h'}]_g}_{h'}}{\\
    & \;\; \for{h'} \\
    & \;\; \;\; \letin{a_{h'}(\ast)(γ^{h'} ⨆ λ)}{\Braket{\vec p | [A(h ↪ h' \,{\textstyle \pushout}_g\, h)(x_h), \, λ^h]_{h'}}_h}{\\
    &  \;\; \;\; \;\; \for{h} \; \\
    &  \;\; \;\; \;\; \;\; \letin{ŋ^{y_{h'}}_{h' \,{\scriptsize \pushout}_g\, h}(A(h ↪ h' \,{\textstyle \pushout}_g\, h)(x_h), h' ↪ h' \,{\textstyle \pushout}_g\, h)(λ^h ⨆ γ^{h'} ⨆ λ)}{\\
    &  \;\; \;\; \;\; \;\; \hspace{10em} 1 ⋅ \Ket{\bigl[(A(h ↪ h' \,{\textstyle \pushout}_g\, h)(x_h), B(h' ↪ h' \,{\textstyle \pushout}_g\, h)(y_{h'})), !\bigr]_h}}{\\
    &  \mkern-25mu \Braket{ \big(q_{h_1'} ⋅ \Bra{\vec p} \quad ⋯ \quad q_{h_m'} ⋅ \Bra{\vec p}\big) | \big[(A(h ↪ h' \,{\textstyle \pushout}_g\, h)(x_h), B(h' ↪ h' \,{\textstyle \pushout}_g\, h)(y_{h'})), λ^h \,⨆\, γ^{h'} \big]_g}_h}}}
\end{align*}

But the equivalence class $\big[(A(h ↪ h' \,{\textstyle \pushout}_g\, h)(x_h), B(h' ↪ h' \,{\textstyle \pushout}_g\, h)(y_{h'})), λ^h \,⨆\, γ^{h'} \big]_g$ has probabilistic weight $p_h q_{h'} =  q_{h'} p_h$ in both formal convex sums (in the first ket, the index ranges of over the $h'$'s for each $h$, and in the second ket, it ranges over the $h$'s for each $h'$), which yields the result. 

\endgroup
\end{proof}


\subsection{Affineness}

\begin{lemma}\label{lemma:T-on-constant-presheaves}
    Let $X$ be a constant presheaf on the coslice category $g/\BiG$, \ie there exists a set $S_0$ such that
    $$X(g \xinjto {ι} h) = S_0 \xto {\id} S_0$$ 
    for every $g \xinjto {ι} h \in g/\BiG$. Then $$T(X)(g) ≅ \Prfin(S_0)^{[0, 1]^{g_L}}$$
\end{lemma}
\begin{proof}
    This results from a small calculation: 

    $$T(X)(g) ≝ \Big(\Prfin \int^{g ↪ h} X(h) × [0, 1]^{(h-g)_L}\Big)^{[0,1]^{g_L}} = \Big(\Prfin \int^{g ↪ h} S_0 × [0, 1]^{(h-g)_L}\Big)^{[0,1]^{g_L}}$$

    But as the functor $S_0 × -$ is left adjoint to $S_0 ⇒ -$ in $\Sets$, it is cocontinuous, so it preserves coends, and: 

    $$\int^{g ↪ h} S_0 × [0, 1]^{(h-g)_L} ≅ S_0 × \underbrace{\int^{g ↪ h} [0, 1]^{(h-g)_L}}_{= \, \displaystyle\colim\limits_{g ↪ h} [0, 1]^{(h-g)_L}}$$
    
    But $\displaystyle\colim\limits_{g ↪ h} [0, 1]^{(h-g)_L} ≅ \{\ast\}$. Indeed, $h = g$ is initial in $g/\BiG$, so it is terminal in the essential image of $[0, 1]^{((-)-g)_L}$ (by precomposition), and the resulting colimit is $[0, 1]^{(g-g)_L} ≅ [0, 1]^{∅} ≅ \{\ast\}$. Therefore, $\int^{g ↪ h} S_0 × [0, 1]^{(h-g)_L} ≅ S_0$ and the result follows.
\end{proof}


\begin{lemma}[Affineness]
    $T$ is affine, \ie $T(1) ≅ 1$, where $1$ is the terminal object of $[\BiG, \Sets]$.
\end{lemma}

\begin{proof}
    By \cref{lemma:T-on-constant-presheaves}, for every $g ∈ \BiG$: $T(1) ≅ \Prfin(\{\ast\})^{[0, 1]^{g_L}} ≅ \{\ast\}$.
\end{proof}

